Mapping DNN Embedding Manifolds for Network Generalization Prediction

Understanding Deep Neural Network (DNN) performance in changing conditions is essential for deploying DNNs in safety critical applications with unconstrained environments, e.g., perception for self-driving vehicles or medical image analysis. Recently, the task of Network Generalization Prediction (NGP) has been proposed to predict how a DNN will generalize in a new operating domain. Previous NGP approaches have relied on labeled metadata and known distributions for the new operating domains. In this study, we propose the first NGP approach that predicts DNN performance based solely on how unlabeled images from an external operating domain map in the DNN embedding space. We demonstrate this technique for pedestrian, melanoma, and animal classification tasks and show state of the art NGP in 13 of 15 NGP tasks without requiring domain knowledge. Additionally, we show that our NGP embedding maps can be used to identify misclassified images when the DNN performance is poor.

==> archive.tex <==
% A common situation in ML is that an internal dataset is available for training and testing a DNN. Then it must be decided whether the DNN is fit to be deployed based on the internal test set without labeled test data from every operating domain. For tasks in unconstrained environments, some changes in distribution are possible between the internal testing domain and the external operating domain. If the DNN is determined to be fit to be deployed, the goal is to make correct predictions on as much of the external operating data as possible and to be able to flag as many incorrect predictions as possible. OOD detection is a related tasks in Deep Learning, but for OOD detection the goal is to refuse to make any predictions on input samples from a new distribution, i.e., the external operating domain. 

% We are interested in making it practical to use DNNs for safety critical tasks in unconstrained environments. 
% Key areas of research to ensure safe DNN performance in changing conditions are 1) Domain Generalization and Robustness, see Section \ref{back:domain_generalization}, 2) OOD Detection, see Section \ref{back:ood}, and 3) Network Generalization Prediction and model selection, see Section \ref{back:ngp}. 
% A key area of research for this  is Domain Generalization and Robustness: training DNNs so that they perform well even in changing conditions, see Section \ref{back:domain_generalization}. A related area of research is identifying OOD samples or learning to abstain from making a prediction when you expect to make a mistake, see Section \ref{back:ood}. To A related area of research is predicting how a DNN will perform in operating domains and selecting an appropriate model, see Section \ref{back:ngp}. 



% \subsection{Support Vector Machines}
% Support Vector Machines (SVMs) are traditional Machine Learning (ML) classification models that find the linear decision boundary to maximize the margin between classes.
% SVMs can be extended to non-linear decision boundaries using kernels, $\phi(x)$ that compute features that are non-linear combinations of the input data $x$. SVMs can be solved in the primal or dual formulation. Solving for the decision boundary in an SVM is a constrained optimization where, unlike training a DNN, you are guaranteed to find the optimal solution.

% \subsection{Applications}
% LSUN: https://arxiv.org/pdf/1506.03365.pdf

% Sample-free white-box out-of-distribution detection for deep learning
% https://openaccess.thecvf.com/content/CVPR2021W/TCV/papers/Begon_Sample-Free_White-Box_Out-of-Distribution_Detection_for_Deep_Learning_CVPRW_2021_paper.pdf

% Natural Adversarial Examples \cite{pedraza2021really}
% Yann LeCun Learning in High Dimension Always Amounts to Extrapolation
% AdaDC: Adaptive Deep Clustering for Unsupervised Domain Adaptation in Person Re-identification
% Beyond Mutual Information: Generative Adversarial Network for Domain Adaptation using Information Bottleneck Constraint
% SOoD: Self-Supervised Out-of-Distribution Detection Under Domain Shift for Multi-Class Colorectal Cancer Tissue Types

% The DNN is tested with the internal test set and the results from the test set are used to determine whether the DNN is suitable to be deployed. But, once the DNN is used in operation, it may be used in situations where the input data is quite differet, e.g., images from a different camera, different physical setup, outside the distribution that was observed in testing.




% \subsection{DNN Embeddings}\label{back:explainability}
% While DNN weights are not interpretable, previous work has investigated the DNN embeddings, i.e., the intermediate outputs from layers in the DNN, to determine if the input is OOD or adversarial, or to infer the confidence of the prediction. 

% There is significant interest in training DNNs that perform well when they are deployed in unconstrained environments. 
% Domain generalization is an area of research that aims to train DNNs that maintain a high level of performance even when the data distribution shifts compared to the training distribution. DNN robustness is a related area of research that aims to train DNNs that can make good predictions even in the presence of image artifacts, e.g., noise. Adversarial attacks address a particularly challenging area of DNN robustness where the noise is specifically added to the image to fool the DNN. 


% \subsection{Decision Trees}
% A Decision Tree is a classical Machine Learning (ML) model that recursively splits the training data based to minimize the uncertainty or Entropy of the data label at the terminal leaf nodes in the tree. Consider data features $X \in R^{NxD}$ with $N$ samples and $D$ dimensional feature vector. In general, the data features can be  The data is labeled $Y \in R^N$. The decision tree $\Tau$.
% The decision tree uses a greedy algorithm to identify the dimension of the input feature and the threshold split to maximize the information gain.

